Rethinking Visual Geo-localization for Large-Scale Applications

Visual Geo-localization (VG) is the task of estimating the position where a given photo was taken by comparing it with a large database of images of known locations. To investigate how existing techniques would perform on a real-world city-wide VG application, we build San Francisco eXtra Large, a new dataset covering a whole city and providing a wide range of challenging cases, with a size 30x bigger than the previous largest dataset for visual geo-localization. We find that current methods fail to scale to such large datasets, therefore we design a new highly scalable training technique, called CosPlace, which casts the training as a classification problem avoiding the expensive mining needed by the commonly used contrastive learning. We achieve state-of-the-art performance on a wide range of datasets and find that CosPlace is robust to heavy domain changes. Moreover, we show that, compared to the previous state-of-the-art, CosPlace requires roughly 80% less GPU memory at train time, and it achieves better results with 8x smaller descriptors, paving the way for city-wide real-world visual geo-localization. Dataset, code and trained models are available for research purposes at https://github.com/gmberton/CosPlace.

==> tables/backbones.tex <==
% \begin{table*}
% \begin{adjustbox}{width=\textwidth}
% \centering
% \begin{tabular}{lcccccccccccccccccccc}
% \toprule
% \multicolumn{1}{c}{\multirow{2}{*}{Method}} & \multicolumn{1}{c}{\multirow{2}{*}{Desc. dim.}} & \multicolumn{3}{c}{Pitts250k} & & \multicolumn{3}{c}{Pitts30k} & & \multicolumn{3}{c}{Tokyo 24/7} & & \multicolumn{3}{c}{MSLS} & & \multicolumn{3}{c}{St Lucia} \\
% \cline{3-5} \cline{7-9} \cline{11-13} \cline{15-17} \cline{19-21} 
% \multicolumn{2}{c}{}
% & R@1  & R@5  & R@10  & & R@1  & R@5  & R@10  & & R@1  & R@5  & R@10  & & R@1  & R@5  & R@10  & & R@1  & R@5  & R@10 \\
% \hline
% ResNet-18     &   32 & 72.9 & 87.5 & 91.6 & & 76.9 & 89.8 & 92.9 &
% & 38.4 & 63.2 & 71.7 & & 63.3 & 76.0 & 80.0 & & 89.4 & 95.5 & 97.1 \\
% ResNet-50     &   32 & 73.6 & 89.2 & 93.0 & & 76.7 & 90.7 & 93.6 &
% & 46.0 & 63.2 & 71.7 & & 68.4 & 79.9 & 83.3 & & 90.8 & 97.1 & 98.3 \\
% ResNet-101    &   32 & 73.5 & 88.6 & 92.8 & & 76.5 & 90.2 & 93.2 &
% & 46.7 & 67.0 & 76.8 & & 70.5 & 81.2 & 84.3 & & 88.8 & 95.9 & 97.7 \\
% \hline
% VGG-16        &   64 & 82.4 & 92.8 & 95.3 & & 83.1 & 92.5 & 94.6 &
% & 59.7 & 78.1 & 85.1 & & 72.2 & 81.8 & 84.9 & & 87.4 & 95.2 & 96.7 \\
% ResNet-18     &   64 & 84.2 & 94.0 & 96.2 & & 84.4 & 93.0 & 95.2 &
% & 59.7 & 77.5 & 84.8 & & 73.9 & 83.0 & 85.9 & & 95.7 & 98.4 & 99.2 \\
% ResNet-50     &   64 & 85.7 & 94.9 & 96.7 & & 86.1 & 94.1 & 95.7 &
% & 69.5 & 84.4 & 89.5 & & 76.6 & 85.8 & 88.3 & & 95.4 & 99.0 & 99.4 \\
% ResNet-101    &   64 & 85.6 & 95.0 & 96.8 & & 85.7 & 94.1 & 95.7 &
% & 64.8 & 81.0 & 85.1 & & 77.3 & 86.0 & 88.1 & & 94.6 & 98.7 & 99.4 \\
% \hline
% VGG-16        &  128 & 87.1 & 95.2 & 96.9 & & 86.5 & 93.8 & 95.5 &
% & 71.4 & 85.1 & 89.2 & & 76.1 & 85.2 & 87.7 & & 91.3 & 95.6 & 97.1 \\
% ResNet-18     &  128 & 88.6 & 96.3 & 97.6 & & 87.7 & 94.4 & 95.8 &
% & 73.0 & 86.7 & 90.8 & & 77.9 & 86.1 & 88.5 & & 97.0 & 98.9 & 99.2 \\
% ResNet-50     &  128 & 88.8 & 95.8 & 97.2 & & 88.5 & 94.6 & 95.9 &
% & 74.9 & 88.9 & 92.1 & & 80.5 & 88.4 & 90.2 & & 96.7 & 99.2 & 99.7 \\
% ResNet-101    &  128 & 89.5 & 96.8 & 98.0 & & 88.6 & 94.7 & 96.1 &
% & 76.2 & 88.3 & 91.7 & & 81.0 & 88.2 & 90.4 & & 97.5 & 99.2 & 99.5 \\
% \hline
% VGG-16        &  256 & 89.0 & 96.2 & 97.5 & & 88.2 & 94.4 & 95.7 &
% & 80.0 & 89.2 & 91.4 & & 78.9 & 86.5 & 89.2 & & 92.3 & 96.3 & 97.7 \\
% ResNet-18     &  256 & 89.7 & 96.9 & 97.9 & & 88.6 & 94.9 & 96.1 &
% & 76.2 & 88.6 & 92.1 & & 79.9 & 87.7 & 89.9 & & 98.0 & 99.5 & 99.7 \\
% ResNet-50     &  256 & 91.0 & 96.9 & 98.3 & & 89.7 & 95.1 & 96.3 &
% & 79.7 & 89.8 & 93.7 & & 83.0 & 90.1 & 91.9 & & 98.1 & 99.7 & 99.8 \\
% ResNet-101    &  256 & 89.8 & 96.8 & 97.9 & & 88.9 & 95.0 & 96.3 &
% & 78.4 & 90.5 & 94.3 & & 83.1 & 90.3 & 91.9 & & 98.4 & 99.6 & 99.7 \\
% \hline
% CCT224        &  384 & 89.1 & 96.3 & 97.9 & & 87.5 & 94.6 & 96.2 &
% & 68.9 & 80.3 & 85.7 & & 76.1 & 84.4 & 86.9 & & 99.2 & 99.9 & 99.9 \\
% CCT384        &  384 & 90.8 & 97.3 & 98.3 & & 88.9 & 95.5 & 96.7 &
% & 76.8 & 87.6 & 90.5 & & 79.4 & 87.0 & 89.0 & & 99.5 & 99.9 & 99.9 \\
% \hline
% VGG-16        &  512 & 89.2 & 96.1 & 97.5 & & 88.6 & 94.4 & 95.7 &
% & 82.5 & 87.6 & 90.8 & & 79.5 & 87.0 & 89.1 & & 94.9 & 97.5 & 98.6 \\
% ResNet-18     &  512 & 89.8 & 96.8 & 97.8 & & 89.0 & 95.2 & 96.1 &
% & 82.6 & 88.3 & 92.1 & & 80.6 & 88.1 & 90.3 & & 98.0 & 99.6 & 99.7 \\
% ResNet-50     &  512 & 91.7 & 97.4 & 98.4 & & 90.2 & 95.5 & 96.5 &
% & 85.1 & 92.4 & 94.0 & & 83.1 & 90.2 & 91.9 & & 98.4 & 99.7 & 99.9 \\
% ResNet-101    &  512 & 91.4 & 97.5 & 98.4 & & 90.1 & 95.3 & 96.4 &
% & 83.2 & 93.3 & 95.6 & & 84.3 & 90.9 & 92.3 & & 98.1 & 99.6 & 99.9 \\
% \hline
% ViT           & 768  & 89.5 & 96.6 & 98.0 & & 87.5 & 94.3 & 96.0 &
% & 71.4 & 84.8 & 87.6 & & 73.4 & 82.6 & 85.5 & & 99.0 & 99.7 & 99.9 \\
% \hline
% ResNet-50     & 1024 & 91.7 & 97.2 & 98.2 & & 90.4 & 95.4 & 96.6 &
% & 82.9 & 91.4 & 94.0 & & 83.6 & 90.3 & 91.9 & & 98.6 & 99.6 & 99.9 \\
% ResNet-101    & 1024 & 91.4 & 97.5 & 98.4 & & 90.1 & 95.5 & 96.6 &
% & 81.9 & 93.3 & 94.0 & & 84.6 & 90.9 & 92.4 & & 98.1 & 99.6 & 99.8 \\
% \hline
% ResNet-50     & 2048 & 91.5 & 97.5 & 98.3 & & 90.4 & 95.7 & 96.5 &
% & 84.1 & 91.7 & 93.7 & & 84.0 & 90.8 & 92.3 & & 98.3 & 99.5 & 99.8 \\
% ResNet-101    & 2048 & 90.8 & 97.3 & 98.4 & & 90.1 & 96.0 & 96.8 &
% & 79.0 & 89.5 & 92.7 & & 84.2 & 90.9 & 92.3 & & 98.3 & 99.7 & 99.9 \\
% \bottomrule
% \end{tabular}
% \end{adjustbox}
% \caption{
% \textbf{Improving the results with more recent backbones \& experimenting with various descriptors dimensionality.} Comparisons of results using {\our} applied to networks with different backbones and different dimensionalities.
% }
% \label{tab:backbones}
% \end{table*}


==> tables/competitors.tex <==

\begin{table*}
\begin{adjustbox}{width=\textwidth}
\centering
\begin{tabular}{lcccccccccccccccccccccc}
\toprule
\multicolumn{1}{l}{\multirow{2}{*}{Method}} & \multicolumn{1}{c}{\multirow{2}{*}{Desc. dim.}} & \multicolumn{1}{c}{\multirow{2}{*}{Train set}} & \multicolumn{2}{c}{Pitts250k} & & \multicolumn{2}{c}{Pitts30k} & & \multicolumn{2}{c}{Tokyo 24/7} & & \multicolumn{2}{c}{MSLS} & & \multicolumn{2}{c}{St Lucia} \\
\cline{4-5} \cline{7-8} \cline{10-11} \cline{13-14} \cline{16-17}
\multicolumn{3}{c}{}
& R@1  & R@5  & & R@1  & R@5  & & R@1  & R@5 &
& R@1  & R@5  & & R@1  & R@5 \\
\hline
NetVLAD \cite{Arandjelovic_2018_netvlad} & 32768 & Pitts30k
& 85.9\footnotesize{$\pm$ 0.3} & 93.6\footnotesize{$\pm$ 0.2} &
& 86.1\footnotesize{$\pm$ 0.1} & 94.1\footnotesize{$\pm$ 0.3} &
& 57.3\footnotesize{$\pm$ 0.8} & 74.4\footnotesize{$\pm$ 0.6} &
& 54.8\footnotesize{$\pm$ 1.1} & 66.6\footnotesize{$\pm$ 1.0} &
& 70.8\footnotesize{$\pm$ 0.5} & 81.8\footnotesize{$\pm$ 0.7} \\
NetVLAD \cite{Arandjelovic_2018_netvlad} & 32768 & MSLS
& 79.7\footnotesize{$\pm$ 0.8} & 90.2\footnotesize{$\pm$ 0.9} &
& 80.9\footnotesize{$\pm$ 1.4} & 90.6\footnotesize{$\pm$ 1.2} &
& 63.6\footnotesize{$\pm$ 1.1} & 77.5\footnotesize{$\pm$ 1.2} &
& 75.4\footnotesize{$\pm$ 0.4} & 84.2\footnotesize{$\pm$ 0.2} &
& 92.8\footnotesize{$\pm$ 0.4} & \textbf{97.6\footnotesize{$\pm$ 0.3}} \\
NetVLAD \cite{Arandjelovic_2018_netvlad} & 32768 & {\ourD}*
& 81.5\footnotesize{$\pm$ 0.1} & 90.8\footnotesize{$\pm$ 0.3} &
& 82.1\footnotesize{$\pm$ 0.2} & 91.5\footnotesize{$\pm$ 0.2} &
& 66.3\footnotesize{$\pm$ 0.4} & 78.2\footnotesize{$\pm$ 0.5} &
& 59.3\footnotesize{$\pm$ 0.8} & 68.7\footnotesize{$\pm$ 0.7} &
& 80.6\footnotesize{$\pm$ 0.5} & 90.7\footnotesize{$\pm$ 0.8} \\
NetVLAD \cite{Arandjelovic_2018_netvlad} & 32768 & {\ourD}**
& 76.2\footnotesize{$\pm$ 0.3} & 88.8\footnotesize{$\pm$ 0.4} &
& 78.8\footnotesize{$\pm$ 0.4} & 90.0\footnotesize{$\pm$ 0.4} &
& 56.2\footnotesize{$\pm$ 0.8} & 67.7\footnotesize{$\pm$ 0.9} &
& 51.4\footnotesize{$\pm$ 0.9} & 60.7\footnotesize{$\pm$ 0.7} &
& 78.5\footnotesize{$\pm$ 0.6} & 88.3\footnotesize{$\pm$ 0.8} \\
CRN \cite{Kim_2017_crn} & 32768 & Pitts30k
& 87.0\footnotesize{$\pm$ 0.4} & 94.5\footnotesize{$\pm$ 0.1} &
& 86.3\footnotesize{$\pm$ 0.4} & 94.6\footnotesize{$\pm$ 0.4} &
& 62.8\footnotesize{$\pm$ 0.5} & 77.4\footnotesize{$\pm$ 0.8} &
& 57.6\footnotesize{$\pm$ 0.3} & 70.4\footnotesize{$\pm$ 0.8} &
& 70.9\footnotesize{$\pm$ 0.7} & 82.8\footnotesize{$\pm$ 0.7} \\
SPE-VLAD \cite{Yu_2020_SPEVlad} \textdagger & 32768 & Pitts30k
&  -   &  -   & &  -   & 89.2 & &  -   & 63.9 &
&  -   &  -   & &  -   &  -   \\
SARE \cite{Liu_2019_sare} &  4096 & Pitts30k
& 88.0\footnotesize{$\pm$ 0.6} & 94.8\footnotesize{$\pm$ 0.3} &
& 87.2\footnotesize{$\pm$ 0.8} & 93.9\footnotesize{$\pm$ 0.3} &
& 74.8\footnotesize{$\pm$ 3.0} & 84.3\footnotesize{$\pm$ 1.6} &
& 62.4\footnotesize{$\pm$ 2.9} & 73.2\footnotesize{$\pm$ 2.8} &
& 72.7\footnotesize{$\pm$ 2.6} & 86.0\footnotesize{$\pm$ 2.0} \\

SFRS \cite{Ge_2020_sfrs} &  4096 & Pitts30k
& \textbf{90.1\footnotesize{$\pm$ 0.3}} & 95.8\footnotesize{$\pm$ 0.2} &
& \textbf{88.7\footnotesize{$\pm$ 0.3}} & 94.2\footnotesize{$\pm$ 0.1} &
& 78.5\footnotesize{$\pm$ 0.8} & 87.3\footnotesize{$\pm$ 0.5} &
& 62.8\footnotesize{$\pm$ 0.8} & 73.0\footnotesize{$\pm$ 0.8} &
& 72.5\footnotesize{$\pm$ 3.6} & 85.4\footnotesize{$\pm$ 3.2} \\
% https://arxiv.org/pdf/2108.08443.pdf
SRALNet \cite{Peng_2021_sralNet} \textdagger & 4096 & Pitts30k
& 87.8 & 94.8 & &  -   &  -   & & 72.1 & 83.2 &
&  -   &  -   & &  -   &  -   \\
% https://openaccess.thecvf.com/content/ICCV2021/papers/Peng_Attentional_Pyramid_Pooling_of_Salient_Visual_Residuals_for_Place_Recognition_ICCV_2021_paper.pdf
APPSVR \cite{Peng_2021_appsvr} \textdagger & 4096 & Pitts30k
& 88.8 & 95.6 & & 87.4 & 94.3 & & 77.1 & 85.7 &
&  -   &  -   & &  -   &  -   \\
\hline
GeM \cite{Radenovic_2019_gem} &   512 & Pitts30k
& 75.3\footnotesize{$\pm$ 0.2} & 88.4\footnotesize{$\pm$ 0.3} &
& 77.9\footnotesize{$\pm$ 0.4} & 90.5\footnotesize{$\pm$ 0.3} &
& 46.4\footnotesize{$\pm$ 0.9} & 65.3\footnotesize{$\pm$ 0.7} &
& 51.8\footnotesize{$\pm$ 0.9} & 64.4\footnotesize{$\pm$ 0.9} &
& 59.9\footnotesize{$\pm$ 1.6} & 76.3\footnotesize{$\pm$ 2.0} \\
GeM \cite{Radenovic_2019_gem} &   512 & MSLS
& 65.3\footnotesize{$\pm$ 1.2} & 81.0\footnotesize{$\pm$ 1.6} &
& 71.6\footnotesize{$\pm$ 2.1} & 85.1\footnotesize{$\pm$ 1.9} &
& 44.9\footnotesize{$\pm$ 1.7} & 62.6\footnotesize{$\pm$ 1.2} &
& 66.7\footnotesize{$\pm$ 0.7} & 78.9\footnotesize{$\pm$ 0.5} &
& 84.6\footnotesize{$\pm$ 1.1} & 93.3\footnotesize{$\pm$ 0.7} \\
GeM \cite{Radenovic_2019_gem} &   512 & {\ourD}*
& 64.7\footnotesize{$\pm$ 0.8} & 81.4\footnotesize{$\pm$ 0.8} &
& 67.8\footnotesize{$\pm$ 0.6} & 83.6\footnotesize{$\pm$ 0.7} &
& 37.9\footnotesize{$\pm$ 2.3} & 51.0\footnotesize{$\pm$ 2.1} &
& 46.8\footnotesize{$\pm$ 2.1} & 58.1\footnotesize{$\pm$ 1.2} &
& 68.5\footnotesize{$\pm$ 2.4} & 82.7\footnotesize{$\pm$ 1.8} \\
NetVLAD \cite{Arandjelovic_2018_netvlad} &   512 & Pitts30k
& 83.7\footnotesize{$\pm$ 0.3} & 92.8\footnotesize{$\pm$ 0.1} &
& 83.0\footnotesize{$\pm$ 0.2} & 92.6\footnotesize{$\pm$ 0.3} &
& 52.6\footnotesize{$\pm$ 1.1} & 70.9\footnotesize{$\pm$ 1.2} &
& 51.1\footnotesize{$\pm$ 1.0} & 63.5\footnotesize{$\pm$ 0.8} &
& 59.8\footnotesize{$\pm$ 0.5} & 74.5\footnotesize{$\pm$ 1.2} \\
NetVLAD \cite{Arandjelovic_2018_netvlad} &   512 & MSLS
& 74.6\footnotesize{$\pm$ 1.3} & 86.8\footnotesize{$\pm$ 1.2} &
& 77.0\footnotesize{$\pm$ 0.9} & 88.6\footnotesize{$\pm$ 1.2} &
& 50.5\footnotesize{$\pm$ 2.2} & 65.1\footnotesize{$\pm$ 1.7} &
& 72.6\footnotesize{$\pm$ 0.5} & 83.0\footnotesize{$\pm$ 0.3} &
& 92.6\footnotesize{$\pm$ 0.6} & 97.1\footnotesize{$\pm$ 0.4} \\
NetVLAD \cite{Arandjelovic_2018_netvlad} &   512 & {\ourD}*
& 77.5\footnotesize{$\pm$ 0.5} & 88.5\footnotesize{$\pm$ 0.2} &
& 79.7\footnotesize{$\pm$ 0.3} & 90.0\footnotesize{$\pm$ 0.4} &
& 53.0\footnotesize{$\pm$ 0.9} & 70.2\footnotesize{$\pm$ 0.5} &
& 53.1\footnotesize{$\pm$ 3.2} & 64.2\footnotesize{$\pm$ 2.2} &
& 78.7\footnotesize{$\pm$ 1.6} & 88.1\footnotesize{$\pm$ 1.8} \\
CRN \cite{Kim_2017_crn} &   512 & Pitts30k
& 84.6\footnotesize{$\pm$ 0.6} & 93.6\footnotesize{$\pm$ 0.3} &
& 84.3\footnotesize{$\pm$ 0.2} & 92.7\footnotesize{$\pm$ 0.2} &
& 53.4\footnotesize{$\pm$ 0.5} & 70.6\footnotesize{$\pm$ 0.8} &
& 54.1\footnotesize{$\pm$ 0.6} & 66.1\footnotesize{$\pm$ 0.6} &
& 56.6\footnotesize{$\pm$ 2.7} & 75.5\footnotesize{$\pm$ 2.9} \\
% https://arxiv.org/pdf/1808.00288.pdf
APANet \cite{Zhu_2018_apanet} \textdagger & 512 & Pitts30k
& 83.7 & 92.6 & &  -   &  -   & & 67.0 & 81.0 &
&  -   &  -   & &  -   &  -   \\
SARE \cite{Liu_2019_sare} &   512 & Pitts30k
& 84.3\footnotesize{$\pm$ 0.7} & 92.6\footnotesize{$\pm$ 0.4} &
& 84.7\footnotesize{$\pm$ 0.7} & 92.6\footnotesize{$\pm$ 0.5} &
& 62.0\footnotesize{$\pm$ 0.6} & 74.9\footnotesize{$\pm$ 0.4} &
& 55.8\footnotesize{$\pm$ 3.3} & 67.8\footnotesize{$\pm$ 3.3} &
& 63.4\footnotesize{$\pm$ 3.0} & 79.0\footnotesize{$\pm$ 1.9} \\
SFRS \cite{Ge_2020_sfrs} &   512 & Pitts30k
& 87.1\footnotesize{$\pm$ 0.4} & 94.6\footnotesize{$\pm$ 0.2} &
& 86.4\footnotesize{$\pm$ 0.5} & 93.8\footnotesize{$\pm$ 0.2} &
& 66.7\footnotesize{$\pm$ 1.0} & 79.6\footnotesize{$\pm$ 0.9} &
& 57.6\footnotesize{$\pm$ 1.1} & 68.9\footnotesize{$\pm$ 1.0} &
& 65.8\footnotesize{$\pm$ 3.1} & 80.1\footnotesize{$\pm$ 2.3} \\
SRALNet \cite{Peng_2021_sralNet} \textdagger & 512 & Pitts30k
& 84.8 & 93.5 & &  -   &  -   & & 60.6 & 76.5 &
&  -   &  -   & &  -   &  -   \\
APPSVR \cite{Peng_2021_appsvr} \textdagger & 512 & Pitts30k
& 85.3 & 94.0 & &  -   &  -   & & 62.0 & 76.5 &
&  -   &  -   & &  -   &  -   \\
\hline
\textbf{{\our} (Ours)} &   512 & {\ourD}
& 89.3\footnotesize{$\pm$ 0.2} & \textbf{96.2\footnotesize{$\pm$ 0.3}} &
& 88.5\footnotesize{$\pm$ 0.1} & \textbf{94.5\footnotesize{$\pm$ 0.2}} &
& \textbf{82.2\footnotesize{$\pm$ 0.5}} & \textbf{88.9\footnotesize{$\pm$ 0.9}} &
& \textbf{79.6\footnotesize{$\pm$ 0.5}} & \textbf{87.2\footnotesize{$\pm$ 0.4}} &
& \textbf{94.1\footnotesize{$\pm$ 0.8}} & 97.4\footnotesize{$\pm$ 0.1} \\
\bottomrule
\end{tabular}
\end{adjustbox}
\caption{\textbf{Comparisons of various methods on popular datasets.} Various values of recalls are used as metric (R@1, R@5), with threshold distance for positives of 25 meters. All results rely on a CNN with a VGG-16 backbone, and are averaged over 3 runs with seeds 0, 1 and 2.
* images taken after 2010 are used as queries, and the rest as database.
** images taken after 2015 are used as queries, and the rest as database.
\textdagger these results could not be independently verified given that no public code implementation is available and we were unable to reproduce the results. The results (when available) were taken from the respective papers.
}
\label{tab:results_recalls}
\vspace{-0.3cm}
\end{table*}



\begin{table}
\begin{adjustbox}{width=\linewidth}
\centering
\begin{tabular}{lccccccccc}
\toprule
\multicolumn{1}{l}{\multirow{2}{*}{Method}} & \multicolumn{1}{c}{\multirow{2}{*}{Desc. dim.}} & \multicolumn{1}{c}{\multirow{2}{*}{Train set}} & \multicolumn{3}{c}{{\ourD} v1} & & \multicolumn{3}{c}{{\ourD} v2} \\
\cline{4-6} \cline{8-10}
\multicolumn{3}{c}{}
& R@1  & R@5  & R@10  & & R@1  & R@5  & R@10 \\
\hline
NetVLAD       & 32768 & Pitts30k
& 40.0 & 48.8 & 52.8 & & 71.1 & 82.4 & 84.8 \\
NetVLAD       & 32768 & MSLS
& 22.9 & 32.0 & 37.1 & & 48.2 & 64.7 & 69.7 \\
NetVLAD       & 32768 & {\ourD}*
& 38.3 & 47.4 & 51.7 & & 70.7 & 83.4 & 87.0 \\
NetVLAD       & 32768 & {\ourD}**
& 28.4 & 38.6 & 43.1 & & 60.9 & 74.6 & 78.6 \\
CRN           & 32768 & Pitts30k
& 45.8 & 56.9 & 60.7 & & 76.4 & 85.3 & 87.8 \\
SARE          &  4096 & Pitts30k
& 45.5 & 56.5 & 60.0 & & 78.8 & 87.6 & 90.5 \\
SFRS          &  4096 & Pitts30k
& 51.2 & 62.2 & 66.6 & & 83.1 & 90.5 & 93.5 \\
\hline
GeM           &   512 & Pitts30k
& 21.7 & 30.3 & 34.4 & & 43.1 & 63.7 & 69.2 \\
GeM           &   512 & MSLS
&  8.1 & 15.6 & 20.2 & & 29.3 & 46.3 & 53.8 \\
GeM           &   512 & {\ourD}*
&  9.8 & 17.6 & 21.2 & & 34.8 & 55.5 & 63.0 \\
NetVLAD       &   512 & Pitts30k
& 27.4 & 38.1 & 43.6 & & 66.7 & 79.3 & 82.9 \\
NetVLAD       &   512 & MSLS
& 14.5 & 21.0 & 28.9 & & 40.5 & 59.7 & 64.4 \\
NetVLAD       &   512 & {\ourD}*
& 25.4 & 32.9 & 40.5 & & 66.9 & 78.6 & 82.8 \\
CRN           &   512 & Pitts30k
& 31.4 & 43.0 & 49.7 & & 68.2 & 81.3 & 83.3 \\
SARE          &   512 & Pitts30k
& 30.8 & 42.1 & 46.5 & & 69.2 & 81.1 & 83.1 \\
SFRS          &   512 & Pitts30k
& 35.6 & 49.7 & 54.8 & & 78.1 & 88.5 & 91.3 \\
\hline
\textbf{{\our} (Ours)} & 512 & {\ourD}
& \textbf{65.1} & \textbf{73.6} & \textbf{77.6} & & \textbf{83.4} & \textbf{92.1} & \textbf{94.8} \\
\bottomrule
\end{tabular}
\end{adjustbox}
\caption{\textbf{Comparisons on {\ourD} v1 and {\ourD} v2.}}
\label{tab:results_recalls_sf_xxl}
\vspace{-0.3cm}
\end{table}

